Efficient Certified Training and Robustness Verification of Neural ODEs

Neural Ordinary Differential Equations (NODEs) are a novel neural architecture, built around initial value problems with learned dynamics which are solved during inference. Thought to be inherently more robust against adversarial perturbations, they were recently shown to be vulnerable to strong adversarial attacks, highlighting the need for formal guarantees. However, despite significant progress in robustness verification for standard feed-forward architectures, the verification of high dimensional NODEs remains an open problem. In this work, we address this challenge and propose GAINS, an analysis framework for NODEs combining three key ideas: (i) a novel class of ODE solvers, based on variable but discrete time steps, (ii) an efficient graph representation of solver trajectories, and (iii) a novel abstraction algorithm operating on this graph representation. Together, these advances enable the efficient analysis and certified training of high-dimensional NODEs, by reducing the runtime from an intractable $O(\exp(d)+\exp(T))$ to ${O}(d+T^2 \log^2T)$ in the dimensionality $d$ and integration time $T$. In an extensive evaluation on computer vision (MNIST and FMNIST) and time-series forecasting (PHYSIO-NET) problems, we demonstrate the effectiveness of both our certified training and verification methods.

==> test-section.tex <==
\section{Test Section} \label{sec:test}

Interesting stuff:

\begin{itemize}
	\item Citations are set up already: Turing~\cite{turing1937computable}
	\item You may use UTF-8 characters: ä
	\item Use cref for references: \cref{sec:test}
	\item Reference the appendix: \cref{fig:appendix} in \cref{app:test-appendix}
	\item Use the \texttt{acro} package for acronyms: First usage: \ac{cli}, subsequent usages: \ac{cli}
\end{itemize}

\begin{figure}[t]
	\centering
	\includegraphics[height=2cm]{example-image-a}
	\caption{An example figure caption.}
	\label{fig:example}
\end{figure}

\paragraph{Figures}
See \cref{fig:example} for an example figure.

\lstinputlisting[float=t,caption={Example code.},label=lst:code]{code/example-code.psi}

\paragraph{Listings}
See \cref{lst:code} for an example Listing.

